Supersymmetry Across the Light and Heavy-Light Hadronic Spectrum II

We extend our analysis of the implications of hadronic supersymmetry for heavy-light hadrons in light-front holographic QCD. Although conformal symmetry is strongly broken by the heavy quark mass, supersymmetry and the holographic embedding of semiclassical light-front dynamics derived from five-dimensional anti-de Sitter (AdS) space nevertheless determines the form of the confining potential in the light-front Hamiltonian to be harmonic. The resulting light-front bound-state equations lead to a heavy-light Regge-like spectrum for both mesons and baryons. The confinement hadron mass scale and their Regge slopes depend, however, on the mass of the heavy quark in the meson or baryon as expected from Heavy Quark Effective Theory (HQET). This procedure reproduces the observed spectra of heavy-light hadrons with good precision and makes predictions for yet unobserved states.

==> definitions.tex <==
%Definitions

\def\Dslash{\raise.15ex\hbox{/}\kern-.7em D}
\def\Pslash{\raise.15ex\hbox{/}\kern-.7em P}


\newcommand{\beq}{\begin{equation}}
\newcommand{\enq}{\end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\beqast}{\begin{eqnarray*}}
\newcommand{\enqa}{\end{eqnarray}}
\newcommand{\enqast}{\end{eqnarray*}}
\newcommand{\nn}{\nonumber}
\newcommand{\req}[1]{(\ref{#1})}
\newcommand{\lb}{\label}
\newcommand{\rf}{\ref}
\newcommand{\ct}{\cite}

\renewcommand{\arraystretch}{1.3}

\newcommand{\cM}{\mathcal{M}}
\newcommand{\mbf}[1]{\mathbf{#1}}


\newcommand{\half}{{\frac{1}{2}}}
 \newcommand{\threehalf}{{\frac{3}{2}}}
 \newcommand{\fivehalf}{{\frac{5}{2}}}
 \newcommand{\sevenhalf}{{\frac{7}{2}}}
 \newcommand{\ninehalf}{{\frac{9}{2}}}
 \newcommand{\elevenhalf}{{\frac{11}{2}}}
 \newcommand{\thirteenhalf}{{\frac{13}{2}}}


\newcommand{\pa}{\partial}


\newcommand{\bec}{\begin{center}}
\newcommand{\enc}{\end{center}}
\newcommand{\beqo}{\begin{quote}}
\newcommand{\enqo}{\end{quote}}
\newcommand{\fn}{\footnote}



\newcommand{\LD}{{\cal L}}
\newcommand{\cL}{{\cal L}}
\newcommand{\Z}{{\cal T}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cD}{{\cal D}}
\newcommand{\cG}{{\cal G}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cC}{{\cal C}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cR}{{\cal R}}
\newcommand{\bA}{\mbox{\bf A}}
\newcommand{\bB}{\mbox{\bf B}}
\newcommand{\bF}{\mbox{\bf F}}
\newcommand{\bG}{\mbox{\bf G}}
\newcommand{\bD}{\mbox{\bf D}}
\newcommand{\bU}{\mbox{\bf U}}
\newcommand{\bV}{\mbox{\bf V}}

\newcommand{\al}{\alpha}
\newcommand{\be}{\beta}
\newcommand{\ga}{\gamma}
\newcommand{\de}{\delta}
\newcommand{\ep}{\epsilon}
\newcommand{\ze}{\zeta}
\newcommand{\et}{\eta}
%\newcommand{\th}{\theta}
\newcommand{\io}{\iota}
\newcommand{\ka}{\kappa}
\newcommand{\la}{\lambda}
\newcommand{\rh}{\rho}
\newcommand{\si}{\sigma}
\newcommand{\varsi}{\varsigma}
\newcommand{\ta}{\tau}
\newcommand{\up}{\upsilon}
\newcommand{\ph}{\phi}
\newcommand{\ch}{\chi}
\newcommand{\ps}{\psi}
\newcommand{\om}{\omega}
\newcommand{\omis}{\omega_{!!!!!!!! \iota}}
\newcommand{\vp}{\varphi}
\newcommand{\Al}{\Alpha}
\newcommand{\Be}{B}
\newcommand{\Ga}{\Gamma}
\newcommand{\De}{\Delta}
\newcommand{\Ep}{E}
\newcommand{\Ze}{Z}
\newcommand{\Et}{H}
\newcommand{\Th}{\Theta}
\newcommand{\Ka}{K}
\newcommand{\La}{\Lambda}
\newcommand{\Rh}{P}
\newcommand{\Si}{\Sigma}
\newcommand{\Ta}{T}
\newcommand{\Up}{\Upsilon}
\newcommand{\Ph}{\Phi}
\newcommand{\Ch}{X}
\newcommand{\Ps}{\Psi}
\newcommand{\Om}{\Omega}





